Better abstractions for timed automata

We consider the reachability problem for timed automata. A standard solution to this problem involves computing a search tree whose nodes are abstractions of zones. These abstractions preserve underlying simulation relations on the state space of the automaton. For both effectiveness and efficiency reasons, they are parametrized by the maximal lower and upper bounds (LU-bounds) occurring in the guards of the automaton. We consider the aLU abstraction defined by Behrmann et al. Since this abstraction can potentially yield non-convex sets, it has not been used in implementations. We prove that aLU abstraction is the biggest abstraction with respect to LU-bounds that is sound and complete for reachability. We also provide an efficient technique to use the aLU abstraction to solve the reachability problem.

==> fig-dist-graph.tex <==
\begin{tikzpicture}
  %%% Graph of (x-y>=1 && y<2 && x>4)
  \begin{scope}[xshift=0cm]
    % Nodes of the graph
    \node (0) at (0,0) {$0$};
    \node (x) at (2,0) {$x$};
    \node (y) at (4,0) {$y$};
    % Edges of the graph
    \begin{scope}[->,thick,>=stealth,bend angle=10]
      \tiny
      \draw (0) edge[bend left] node[above] {$(<,\infty)$} (x);
      \draw[rounded corners] (0.south) |- (2,-0.5) node[below]
      {$(<,2)$} -| (y.south);
      \draw (x) edge[bend left] node[below] {$(<,-4)$} (0);
      \draw (x) edge[bend left] node[above] {$(\le, -1)$} (y);
      \draw (y) edge[bend left] node[below] {$(<,\infty)$} (x);
      \draw[rounded corners] (y.north) |- (2,0.5) node[above]
      {$(<,\infty)$} -| (0.north);
    \end{scope}
  \end{scope}
\end{tikzpicture}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "m"
%%% End: 


==> fig/nonconvex-algo.tex <==
{
  % \setlength{\columnsep}{35pt}
  % \setlength{\columnseprule}{0.5pt}
  \begin{lstlisting}[mathescape=true, float=t, columns=fullflexible,
    caption={ Reachability algorithm to incorporate non-convex abstractions
      $\abssim$ based on time-abstract simulation}, label=fig:non_convex_algorithm]
    function main() 
    
    Waiting := $\emptyset$;
    Visited := $\emptyset$;

    Add $(q_0,Z_0)$ to Waiting

    while (Waiting $\neq$ $\es$) 
         Remove $(q,Z)$ from Waiting;
         if ($q$ is accepting) 
             exit $\mathit{Yes}$ 
         else if ( $\exists$ $(q,Z') \in$ Visited s.t. $\mathbf{Z
           \incl \abssim(Z')}$ ) 
             continue 
         else 
          for each $(q_s,Z_s)$ s.t. $(q,Z) \tto (q_s,
          Z_s)$ do
              if ($Z_s$ $\neq$ $\es$)
                  Add ($q_s,Z_s)$ to Waiting
 
    return $\mathit{No}$
  \end{lstlisting}
}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../m"
%%% End: 

